Anomaly Factory 3D: A Modular Framework for Diverse Pseudo-Anomaly Synthesis in Unsupervised 3D Anomaly Detection

Detecting and localizing defects in 3D point clouds is challenging because abnormal samples are scarce and diverse, while training is often limited to normal data. We propose Anomaly Factory 3D (AF3AD), a modular framework that synthesizes diverse pseudo-anomalies from normal point clouds to expand the training data for unsupervised 3D anomaly detection methods that rely on pseudo-anomalies. AF3AD uses a center-conditioned parametric deformation model defined in local PCA frames, with kernel-controlled spatial falloff, anisotropy, directional gating, and normal/tangential displacement fields, enabling a broad set of geometric defect presets. We demonstrate its ease-of-use and effectiveness by integrating AF3AD with an offset-prediction detector and a reconstruction-based anomaly detection method, showing that AF3AD transfers across detection paradigms. Experiments on AnomalyShapeNet and Real3D-AD show consistent improvements in object- and point-level detection and localization, supported by ablations on preset groups and robustness under noise. AF3AD is designed as a standalone synthesis tool to facilitate adoption across different 3D anomaly detection paradigms. Code is available at github.com/vpc-ccg/AF3AD.

==> tables/offset_head_ablation.tex <==
\begin{table}[t]
\centering
\caption{Average AUROC across 15 classes of AnomalyShapeNet. We compare the baseline offset head (PO3AD-style) and a multi-head variant under both the PO3AD anomaly generator (Norm-AS) and the proposed generator (AF3AD).}
\label{tab:ablation_arch_avg_aucroc}
\begin{tabular}{lccc}
\toprule
Setting & O-AUROC $\uparrow$ & P-AUROC $\uparrow$ & (O+P)/2 $\uparrow$ \\
\midrule
\multicolumn{4}{l}{\textbf{Norm-AS (PO3AD)}} \\
Baseline (h=32)    & 0.5582 & 0.5569 & 0.5575 \\
Baseline (h=64)    & 0.5509 & 0.5641 & 0.5575 \\
Baseline (h=128)   & 0.5522 & 0.5697 & 0.5610 \\
Multi-head (h=32)  & 0.5733 & 0.5957 & 0.5845 \\
Multi-head (h=64)  & 0.6543 & 0.6332 & 0.6438 \\
Multi-head (h=128) & 0.6638 & 0.6446 & 0.6542 \\
\midrule
\multicolumn{4}{l}{\textbf{AF3AD (ours)}} \\
Baseline (h=32)    & 0.8225 & 0.7988 & 0.8107 \\
Baseline (h=64)    & 0.8285 & 0.8046 & 0.8166 \\
Baseline (h=128)   & 0.8442 & 0.8075 & 0.8258 \\
Multi-head (h=32)  & 0.8773 & 0.8721 & 0.8747 \\
Multi-head (h=64)  & \textbf{0.9118} & \underline{0.8928} & \underline{0.9023} \\
Multi-head (h=128) & \underline{0.9101} & \textbf{0.8947} & \textbf{0.9024} \\
\bottomrule
\end{tabular}
\end{table}

